Rolling Colors: Adversarial Laser Exploits against Traffic Light Recognition

Traffic light recognition is essential for fully autonomous driving in urban areas. In this paper, we investigate the feasibility of fooling traffic light recognition mechanisms by shedding laser interference on the camera. By exploiting the rolling shutter of CMOS sensors, we manage to inject a color stripe overlapped on the traffic light in the image, which can cause a red light to be recognized as a green light or vice versa. To increase the success rate, we design an optimization method to search for effective laser parameters based on empirical models of laser interference. Our evaluation in emulated and real-world setups on 2 state-of-the-art recognition systems and 5 cameras reports a maximum success rate of 30% and 86.25% for Red-to-Green and Green-to-Red attacks. We observe that the attack is effective in continuous frames from more than 40 meters away against a moving vehicle, which may cause end-to-end impacts on self-driving such as running a red light or emergency stop. To mitigate the threat, we propose redesigning the rolling shutter mechanism.

==> sections/attack_model.tex <==
% !TEX root = ../LaserAttack.tex

\section{Laser Attack on Traffic Light Models}

\textbf{Research question:} How can a tainted image under laser attack affect the results of traffic light detection and recognition.

% Send the tainted images to the model and show the results.

During the previous test we find that laser attack is a convenient method to change the color of the image captured by rolling shutter camera. While the traffic light recognition algorithm based on computer vision mainly used the color information in the image. Which means laser attack could be an efficient way to spoof the traffic light recognition algorithm. 

There are two major types of algorithm

% structure of algorithm in the background ????
% 高精度地图给出大致方位(可假定已知)->检测较大范围内是否有红绿灯->将红绿灯框选并送到识别网络识别
% 
% two major types of the algorithm: based on classifier(treat three light as different objects), based on object detector (crop and recognize); two recognition method: traditional CV (color channel), and machine learning (RetinaNET)

\subsection{Impact on Traffic Light Detection}
% 目标: 尽可能不影响Detection
% Dos or no impact
% 亮度过高或者噪点过多会引起Dos, 降低亮度会降低影响
We use yolo as our object detector and test it under

\subsection{Impact on Traffic Light Recognition}
% 基于传统CV: 色彩通道统计, 十分有效
% 基于深度学习: 可能不会十分有效

"traffic-light-classifier" transformed the color in RGB space to HSV space to extract features. It creates mask for green, red, and yellow pixels. The final classification outcome is determined by the total pixels in each mask. By injecting red laser to create more reddish pixels can spoof this algorithm to recognize the traffic light as red light. 
% 两张图...? HSV示意图?

RetinaNet used by Apollo, can be spoofed but more difficult. 
% 但是不知道原理, 直接放图? 

